Enhancing MR Image Segmentation with Realistic Adversarial Data Augmentation

The success of neural networks on medical image segmentation tasks typically relies on large labeled datasets for model training. However, acquiring and manually labeling a large medical image set is resource-intensive, expensive, and sometimes impractical due to data sharing and privacy issues. To address this challenge, we propose AdvChain, a generic adversarial data augmentation framework, aiming at improving both the diversity and effectiveness of training data for medical image segmentation tasks. AdvChain augments data with dynamic data augmentation, generating randomly chained photo-metric and geometric transformations to resemble realistic yet challenging imaging variations to expand training data. By jointly optimizing the data augmentation model and a segmentation network during training, challenging examples are generated to enhance network generalizability for the downstream task. The proposed adversarial data augmentation does not rely on generative networks and can be used as a plug-in module in general segmentation networks. It is computationally efficient and applicable for both low-shot supervised and semi-supervised learning. We analyze and evaluate the method on two MR image segmentation tasks: cardiac segmentation and prostate segmentation with limited labeled data. Results show that the proposed approach can alleviate the need for labeled data while improving model generalization ability, indicating its practical value in medical imaging applications.

==> 0_a_highlights.tex <==
%% Highlights: Highlights should be submitted in a separate editable file in the online submission system. Please
% use 'Highlights' in the file name and include 3 to 5 bullet points (maximum 85 characters, including
% spaces, per bullet point).
\section*{Highlights}
\begin{itemize}
\item A generic, practical adversarial data augmentation framework (\advchain) to better leverage labeled and unlabeled data for medical image segmentation tasks.
\item Unlike conventional adversarial data augmentation with a fixed type of transformation, \advchain\ applies adversarial training to optimizing dynamic compositions of photo-metric and geometric transformations including diffeomorphic deformations to enhance data diversity and effectiveness, generating hard examples with realistic data variations to benefit training.
\item \advchain\ is computationally efficient, where the data augmentation module can be used as a plug-in module to support both supervised and semi-supervised learning even when labeled data is very limited.
\end{itemize}



% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/images/graphical_abstract.pdf}
%     \label{fig:abstract_pdf}
% \end{figure*}

==> 4_exp_adv_chain_vs_adv_compose.tex <==
%% !!this section has been removed for clarity
\subsection{The effectiveness of the chain strategy for adversarial data augmentation}
\label{SEC:Combination vs chain in adversarial data augmentation}
\todo{add p-value test}
\input{tables/random_combination_vs_random_chain}
First, we implemented and compared two different strategies of combining different image transformation functions: \emph{combination} and \emph{chain}, and applied adversarial training to optimizing underlying transformation parameters. These two approaches are denoted as \advcomb\ and \advchain, respectively. Specifically, for \advcomb, adversarial optimization is performed on \emph{each} selected image transformation individually and the network is regularized with optimized transformations using Eq.~\ref{eq:adv comb loss}. For \advchain, the adversarial optimization is performed on a chain of adversarial transformations jointly, as described in Algorithm~\ref{alg1}. The network is regularized with optimized chained transformation using Eq.~\ref{eq:adv chain loss}.
The model performances on the cardiac and the prostate segmentation tasks with different data settings are listed in Table \ref{tab:adv combination vs adv chain}. Results strongly suggest that \advchain\ outperforms \advcomb.

Compared to \advcomb, \advchain\ has  two main advantages. One is that augmented samples with chained transformations exhibit higher diversity. Given $4$ basic image augmentation operations, there are 64 ($4!/3! + 4!/2! + 4!/1! + 4!$) possible ways to chain these transformation operations; whereas there are 15 ($4!/3! +  4!/(2! 
\times 2!) + 4!/(3! 
\times 1!) + 4!/4!$) unique combinations when adopting the combination strategy. This increased data diversity with \advchain\ accounts for the effectiveness in improving the model's generalization ability. In addition, for adversarial data augmentation, performing \advchain\ is more computationally efficient, as it requires less training time. For a random set of $l$  transformations, \advcomb\ requires two forward passes (1 for inner adversarial optimization, 1 for outer network optimization) for each operation, resulting in 2$l$ passes in total. By contrast, \advchain\ only requires two passes for an arbitrary chain and the gradients for each operation can be computed within one backward pass using the chain rule. Therefore, we use \advchain\ as the default way to augment our data for all the experiments below.


==> 6_novelty_statement.tex <==
%% 300 char.
% To the best of our knowledge, the proposed adversarial data augmentation method is the first that designs and constructs realistic adversarial attacks in medical imaging, with the aim of improving the generalization and robustness of MR segmentation networks. The proposed method has three main advantages: 1) high effectiveness to the lack of labelled data; 2) better segmentation robustness on unseen pathological cases; 3) lower computational cost compared to GAN-based methods.

==> check_list.tex <==
guide for authors: 
ref: https://www.elsevier.com/wps/find/journaldescription.cws_home/620983?generatepdf=true

\subsecion{Checklist}
% Manuscript:
• Include keywords (maximum six keywords, american english)
• All figures (include relevant captions)
• All tables (including titles, description, footnotes)
• Ensure all figure and table citations in the text match the files provided
** Indicate clearly if color should be used for any figures in print
Graphical Abstracts / Highlights files (where applicable)
Supplemental files (where applicable)


\subsecion{Highlights}
Highlights are mandatory for this journal as they help increase the discoverability of your article via
search engines. They consist of a short collection of bullet points that capture the novel results of
your research as well as new methods that were used during the study (if any). Please have a look
at the examples here: example Highlights.
Highlights should be submitted in a separate editable file in the online submission system. Please
use 'Highlights' in the file name and include 3 to 5 bullet points (maximum 85 characters, including
spaces, per bullet point).

\subsecion{abstract}
A concise and factual abstract is required. The abstract should state briefly the purpose of the
research, the principal results and major conclusions. An abstract is often presented separately from
the article, so it must be able to stand alone. For this reason, References should be avoided, but if
essential, then cite the author(s) and year(s). Also, non-standard or uncommon abbreviations should
be avoided, but if essential they must be defined at their first mention in the abstract itself.
Graphical abstract
A graphical abstract is mandatory for this journal. It should summarize the contents of the article in
a concise, pictorial form designed to capture the attention of a wide readership online. Authors must
provide images that clearly represent the work described in the article. Graphical abstracts should be
submitted as a separate file in the online submission system. Image size: please provide an image
with a minimum of 531 × 1328 pixels (h × w) or proportionally more. The image should be readable
at a size of 5 × 13 cm using a regular screen resolution of 96 dpi. Preferred file types: TIFF, EPS, PDF
or MS Office files. You can view Example Graphical Abstracts on our information site.
Authors can make use of Elsevier's Illustration Services to ensure the best presentation of their images
also in accordance with all technical requirements.

\subsecion{Figures}
You are urged to visit this site; some excerpts from the detailed information are given here.
Formats
If your electronic artwork is created in a Microsoft Office application (Word, PowerPoint, Excel) then
please supply 'as is' in the native document format.
Regardless of the application used other than Microsoft Office, when your electronic artwork is
finalized, please 'Save as' or convert the images to one of the following formats (note the resolution
requirements for line drawings, halftones, and line/halftone combinations given below):
EPS (or PDF): Vector drawings, embed all used fonts.
TIFF (or JPEG): Color or grayscale photographs (halftones), keep to a minimum of 300 dpi.
TIFF (or JPEG): Bitmapped (pure black & white pixels) line drawings, keep to a minimum of 1000 dpi.
TIFF (or JPEG): Combinations bitmapped line/half-tone (color or grayscale), keep to a minimum of
500 dpi

==> figures/DA_composition.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/images/DA_composition.png}
    \caption{Illustration of augmenting data with a random subset of transformation using different strategies: a) combination; b) chain (the proposed). Here, the transformations with solid lines are selected transformations for data augmentation at one iteration. The probability of selecting each operation is $0.5$. Best viewed in color.}
    \label{fig:DA_composition}
\end{figure*}

==> figures/adv_example.tex <==
In our experiments, \begin{figure*}[t]
    \centering
    \includegraphics[height=0.3\textheight]{figures/images/adv_example.png}
    \caption{Visualization of generated adversarial examples and failed network predictions on  cardiac images (a)-(c) and prostate images (d)-(f) during training. Before/After: network prediction before/after adversarial (adv) attacks. Best viewed in color.}
    \label{fig:adv_example}
\end{figure*}

==> figures/adv_vs_rand_figure.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/images/adv_vs_rand.png}
    \caption{(a-b) Visualization of augmented images with random bias field and adversarial bias field after one-step optimization;(c-d) 
    Augmented examples and network predictions with random deformation and adversarial deformation after one-step optimization. Top blocks show results on cardiac images whereas bottom blocks are results on prostate images. Best viewed in color.}
    \label{fig:adv_example_vs_rand_example}
\end{figure*}
\todo{add one more figure with prostate}

==> figures/tmi_example.tex <==
%  When submitting your final paper, your graphics should all be submitted in- dividually in one of these formats (s PostScript (PS), Encapsulated PostScript (.EPS), Tagged Image File Format (.TIFF), Portable Document Format (.PDF), Portable Network Graphics (.PNG), or Metapost (.MPS)) along with the manuscript.

% The online tool, located at http://graphicsqc.ieee.org/, allows authors to upload their graphics in order to check that each file is the correct file format, resolution, size and colorspace; that no fonts are 
 
%%Most charts, graphs, and tables are one column wide (3.5 inches/88 millimeters/21 picas) or page wide (7.16 inches/181 millimeters/43 picas). The maximum depth a graphic can be is 8.5 inches (216 millimeters/54 picas). When choosing the depth of a graphic, please allow space for a caption. Figures can be sized between column and page widths if the author chooses, however it is recommended that figures are not sized less than column width unless when necessary.

%%Labels should appear centered below each subfigure in 8 point Times New Roman font in the format of (a) (b) (c).


==> figures/varying_different_length.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figures/images/different_length.png}
    \caption{Best viewed in color.}
    \label{fig:varying_different_length}
\end{figure*}

==> tables/random_aug.tex <==
\begin{table}[!ht]
\centering
\caption{\textbf{Segmentation accuracy of U-net trained with different \emph{random} data augmentation strategies in extremely low-data settings.} Reported values are average Dice scores for the left ventricular myocardium segmentation over 20 test subjects. Results with highest scores are represented by bold font.}
\label{tab:random}
\begin{tabular}{@{}lcccrr@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Spatial \\ Aug\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Morph \\ Aug\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Appearance\\ Aug\end{tabular}} & \multicolumn{2}{r}{\# Training subjects} \\ \cmidrule(l){5-6} 
 &  &  &  & 1 & 3 \\ \midrule
Plain &  &  &  & 0.293 & 0.544 \\
Affine & \yesmark &  &  & 0.467 & 0.779 \\
Affine+Intensity & \yesmark &  & \yesmark & 0.536 & 0.797 \\
Affine+Elastic & \yesmark & \yesmark &  & 0.439 & 0.799 \\
Affine+Bias & \yesmark &  & \yesmark & \textbf{0.618} & \textbf{0.808} \\ \bottomrule
\end{tabular}
\end{table}

==> tables/random_combination_vs_random_chain.tex <==
\begin{table}[!ht]
\caption{Adversarial training with simple linear combination (\advcomb) vs chain strategy(\advchain). N: number of labeled subjects, M: number of unlabeled subjects. Reported values are average Dice scores.}
\label{tab:adv combination vs adv chain}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
\multirow{2}{*}{}  & \multicolumn{2}{c|}{Cardiac} & \multicolumn{2}{c}{Prostate} \\
                   & N=1, M=25    & N=3, M=25    & N=3, M=11     & N=11, M=11    \\ \midrule
\advcomb & 0.4705       & 0.7931       & 0.6390        & 0.7279        \\
\advchain      & \textbf{0.5464}      & \textbf{0.8107}       & \textbf{0.6480}    & \textbf{0.7315}   \\ \bottomrule

\end{tabular}
}
\end{table}

==> tables/semi_supervised.tex <==
% \begin{table}[t]
% \centering
% \caption{SSL results on the ACDC dataset under low-shot semi-supervised setting where 25 unlabelled subjects were included during training. Reported values are average Dice scores for each class.}
% \label{tab:acdc_semi_supervised_learning}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}c|ccc|ccc@{}}
% \toprule
%  & \multicolumn{3}{c|}{1 labelled subject} & \multicolumn{3}{c}{3 labelled subjects} \\
%  & LV & MYO & RV & LV & MYO & RV \\ \midrule
% % Baseline &  &  &  &  &  &  \\ \midrule
% Mixup~\citep{Zhang_2018_ICLR_mixup} & 0.5638  & 0.4735 & 0.2769  & 0.8395 & 0.8111 & 0.6795  \\
% VAT~\citep{Miyato_2018_PAMI_VAT} &  0.3893 &  0.2693 &   0.1475   & 0.8557 &   0.8148   & 0.6290 \\
% VAT+EntMin~\citep{Grandvalet_2005_EntropyMinimization} & 0.4657  & 0.3686 & 0.1667 &0.8401   &  0.7974   & 0.6323  \\
% % Rand noise+Mean Teacher~\citep{cui_2019_semi_noise}&   &  &  &  &   & \\
% % Rand Transformation+Self Ensembling~\citep{Li_2020_TNNLS_transformation} &   &  &  &  \\
% Mixmatch~\citep{berthelot_2019_mixmatch} & 0.5582 & 0.4832  &  0.2555 &   0.8518 &  0.8193 &  0.6918 \\
% \midrule
% Rand Compose+EntMin & 0.6759 & 0.5371  & 0.2695 & 0.8613 & 0.8216 & 0.7148 \\
% Adv Compose (w. Adv noise) & 0.6786 &  \textbf{0.5836} &  0.3227 & 0.8545&   0.8245 &   0.7073\\ 
% Adv Compose+EntMin (w. Adv noise) &  \textbf{0.6848} & {0.5808} & \textbf{0.3486} & \textbf{0.8671} & \textbf{0.8333} & \textbf{0.7281}\\ 
% \midrule
% Upperbound & 0.8987 & 0.8563  & 0.7409 & 0.8954 & 0.8619 & 0.7652\\
% % GAN\citep{Chaitanya_2019_IPMI} &
% % 0.834* & 0.710*  & 0.651* &  0.922* & 0.823*  & 0.832* \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
\centering
\caption{SSL results on the ACDC dataset under low-shot semi-supervised setting where 25 unlabeled subjects were included during training. Reported values are average Dice scores for each class.*: images from the unlabeled set are used as labeled images.}
\label{tab:acdc_semi_supervised_learning}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|ccc|ccc@{}}
\toprule
 & \multicolumn{3}{c|}{N=1, M=25} & \multicolumn{3}{c}{N=3, M=25} \\
 & LV & MYO & RV & LV & MYO & RV \\ \midrule
% Baseline &  &  &  &  &  &  \\ \midrule
% Mixup~\citep{Zhang_2018_ICLR_mixup} & 0.5581 & 0.4349 & 0.2017 & 0.8403 & 0.8088 & 0.6705 \\
% Mixmatch~\citep{berthelot_2019_mixmatch} & 0.5220 & 0.4318 & 0.2082 & 0.8534 & 0.8166 & 0.6731 \\

Mixmatch~\citep{berthelot_2019_mixmatch} & 0.6105 & 0.4598 & 0.2529 & 0.8345 &  0.8116 & 0.6608 \\
% Mean-Teacher~\citep{cui_2019_semi_noise} & 0.6078 & 0.4956 & 0.2688 & 0.8551 & 0.7874 & 0.6414 \\
TCSM~\citep{Li_2020_TNNLS_transformation} & 0.6351 & 0.5191 & 0.3238  & 0.8385 & 0.8116 & 0.6751 \\
VAT~\citep{Miyato_2018_PAMI_VAT}& 0.6567 & 0.5464 & 0.3309   & 0.8479 &  0.8284 &  0.6605 \\
\midrule
% \textit{Adv Bias}~\citep{chen_2020_realistic} & \textbf{0.7022}  &  \textbf{0.6329} &  \textbf{0.4272} &  0.8433 &  0.8159 &   0.6971\\
\randchain & 0.6458 & 0.5242 & 0.3472
& 0.8454 & 0.8137 & 0.7223 \\
\advchain & \textbf{0.6878}  & \textbf{0.5686 } & \textbf{0.3827}
& \textbf{0.8650} & \textbf{0.8337} & \textbf{0.7333} \\ \midrule
$\textrm{Upperbound}^*$ & 0.8987 & 0.8563 & 0.7409 & 0.8954 & 0.8619 & 0.7652 \\
\bottomrule
\end{tabular}%
}
\end{table}




% \begin{table}[t]
% \centering
% \caption{SSL results on the prostate dataset under low-shot data setting, where 11 unlabelled subjects were included during training. PZ: peripheral zone; CZ: central zone. Reported values are average Dice scores for each class.}
% \label{tab:prostate_semi_supervised learning}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc@{}}
% \toprule
%  & \multicolumn{2}{c|}{3 labeled subjects} & \multicolumn{2}{c}{11 labeled subjects} \\
%  & PZ & CZ & PZ & CZ \\ \midrule
% % Lower bound &  &  &  &  \\ \midrule
% Mixup~\citep{Zhang_2018_ICLR_mixup} & 0.3152  &    0.6371 & 0.5241 & 0.8076  \\ 
% VAT~\citep{Miyato_2018_PAMI_VAT}& 0.3044 &0.6288 &0.5360  &0.8075 \\
% VAT~\citep{Miyato_2018_PAMI_VAT}+EntMin~\citep{Grandvalet_2005_EntropyMinimization}& 0.3382 &  0.7367 &  0.5336  &  0.8196 \\
% % Rand noise+Mean Teacher~\citep{cui_2019_semi_noise}&   &  &  &  \\
% % Rand Transformation+Self Ensembling~\citep{Li_2020_TNNLS_transformation} &   &  &  &  \\
% Mixmatch~\citep{berthelot_2019_mixmatch} & 0.3883 & 0.6901 & 0.5800  &  0.8204 \\
% \midrule
% Rand Compose+EntMin~& 0.3711    &   0.7172 & & \\
% Adv Compose (w.Adv noise) &  &  &     &   \\ 
% Adv Compose+EntMin (w. Adv noise) & 0.4087 & 0.7408  &0.5838 &  0.8291  \\
% Adv Compose+EntMin (w. Rand noise) &  &   & &\\ 
% \midrule
%  Upperbound  &0.5632   &   0.7863 & {0.6256} & 0.8110 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
\centering
\caption{SSL results on the prostate dataset under low-shot data setting, where 11 unlabeled subjects were included during training. PZ: peripheral zone; CZ: central zone. Reported values are average Dice scores for each class. *: images from the unlabeled set are used as labeled images.}
\label{tab:prostate_semi_supervised learning}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|cc@{}}
\toprule
 & \multicolumn{2}{c|}{N=3, M=11} & \multicolumn{2}{c}{N=11, M=11} \\
 & PZ & CZ & PZ & CZ \\ \midrule
% Lower bound &  &  &  &  \\ \midrule
Mixmatch~\citep{berthelot_2019_mixmatch} & 0.3938 & 0.6966 & 0.5694  & 0.8026  \\
TCSM~\citep{Li_2020_TNNLS_transformation} & 0.4813 & 0.7520 & 0.5938 & 0.8300 \\
VAT~\citep{Miyato_2018_PAMI_VAT} & 0.4622 & 0.7361  &  0.5402 &  0.8051 \\

Fixmatch~\citep{} & 0.4622 & 0.7361  &  0.5402 &  0.8051 \\
% Mean-Teacher~\citep{cui_2019_semi_noise} & 0.3251 & 0.5843 & 0.4817 & 0.7716 \\
\midrule
% \textit{Adv Bias}~\citep{chen_2020_realistic} & 0.4566  & 0.7237  & 0.5464 &  0.8027 \\
\randchain & 0.4991 & 0.7596 & 0.6098 & 0.8300 \\
\advchain & \textbf{0.5216} & \textbf{0.7744} & \textbf{0.6307} & \textbf{0.8322} \\ \midrule
$\textrm{Upperbound}^*$ & 0.5582  & 0.7686 & 0.6249 & 0.8251 \\ \bottomrule
\end{tabular}
}
\end{table}




==> todo_list.tex <==
Based on these reviews, I therefore have the pleasure of accepting it for publication in the Medical Image Analysis Journal, subject to minor revisions. I would like you to send a final version to me including as many of the reviewers' propositions for improvement as possible together with a letter explaining which changes have been made in response to the suggestions from the reviewers (or why you believe no change is required). The modifications must clearly appear in the revised manuscript, using color or boldface for instance. This final version should follow the Medical Image Analysis Guide for Author Electronic format requirements for accepted articles http://www.elsevier.com/wps/find/journaldescription.authors/620983/authorinstructions.

Todo:
figures: https://app.diagrams.net/#G1Keq6px5qqhIuhQLLLvGOOpDm2v1gXukF
Done:
We have revised the manuscripts, according to the suggestions from R4. Major changes are listed below:
* Line 77, we have changed "1 or three labeled subject" to "1 or 3 labeled subjects"
* Line 615, we have deleted the duplicate sentence "To ensure the generated variations to be realistic … which is a common practice".
* Line 1023, we have changed "Adv chain" to "AdvChain"
* Figures 1,4,6,7,9 have been regenerated using PDF format for optimized quality. 

